Characterizing the Complexity of Social Robot Navigation Scenarios

Social robot navigation algorithms are often demonstrated in overly simplified scenarios, prohibiting the extraction of practical insights about their relevance to real-world domains. Our key insight is that an understanding of the inherent complexity of a social robot navigation scenario could help characterize the limitations of existing navigation algorithms and provide actionable directions for improvement. Through an exploration of recent literature, we identify a series of factors contributing to the complexity of a scenario, disambiguating between contextual and robot-related ones. We then conduct a simulation study investigating how manipulations of contextual factors impact the performance of a variety of navigation algorithms. We find that dense and narrow environments correlate most strongly with performance drops, while the heterogeneity of agent policies and directionality of interactions have a less pronounced effect. Our findings motivate a shift towards developing and testing algorithms under higher-complexity settings.

==> packages.tex <==
\usepackage{amssymb, amsmath}
\DeclareMathOperator{\sign}{sign}
\usepackage[sort&compress,numbers,sectionbib]{natbib}
\usepackage{cite} % Compacts [1]--[4] citations and adds spaces
\usepackage{booktabs}
\usepackage[font=footnotesize]{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\renewcommand\thesubfigure{\alph{subfigure}}
\usepackage{verbatimbox}
\usepackage{multirow}
%\usepackage[letterpaper, left=48pt, right=48pt, top=57pt, bottom=43pt]{geometry}

%\usepackage{amsmath,amsfonts}
%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{array}
\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\usepackage{textcomp}
%\usepackage{stfloats}
%\usepackage{url}
%\usepackage{verbatim}
%\usepackage{graphicx}
%\usepackage{cite}
\hyphenation{op-tical net-works semi-conduc-tor IEEE-Xplore}

 \newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.25\textheight][c]{0.8\linewidth}
      \centering{#1}
    \end{minipage}
  }
}

\usepackage{dsfont}

% Labels in IEEE format
% Equation
\newcommand{\eref}[1]{(\ref{#1})}
% Section
\newcommand{\secref}[1]{Sec.~\ref{#1}}
% Figure
\newcommand{\figref}[1]{Fig.~\ref{#1}}
% Table - added
\newcommand{\tabref}[1]{Table~\ref{#1}}


\usepackage[hyphens]{url}

% Insert hyperlinks in the document
\usepackage{hyperref}
\hypersetup{bookmarksopen,bookmarksnumbered,
pdfpagemode=UseOutlines,
colorlinks=true,
linkcolor=teal,
anchorcolor=teal,
citecolor=teal,
filecolor=teal,
menucolor=teal,
urlcolor=teal,
breaklinks=true
}
\urlstyle{same}

%\usepackage[hidelinks]{hyperref}
%\hypersetup{breaklinks=true}
%\usepackage{cite}

\newtheorem{definition}{Definition}[section]
\newtheorem{property}{Property}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{propose}{Proposition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}

% comments
% \def\hidenotes
\usepackage[dvipsnames]{xcolor}
\definecolor{myred}{RGB}{215,48,39}
\definecolor{myblue}{RGB}{69,117,180}
\definecolor{myorange}{RGB}{252,141,89}
\definecolor{mylightblue}{RGB}{145,191,219}


\definecolor{MYlightblue}{RGB}{217,95,2} 
\definecolor{MYdarkblue}{RGB}{117,112,179} 
\definecolor{MYgreen}{RGB}{27,158,119} 








\usepackage{color,soul}
\usepackage{svg}
\newcommand{\cmnote}[1]{{\xxnote{CM}{red}{#1}}}
\newcommand{\xxnote}[3]{}
\ifx\hidenotes\undefined
  \usepackage{color}
  \renewcommand{\xxnote}[3]{\color{#2}{#1: #3}}
\fi

% Enable strikethrough for drafts with /sout{}
\usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}
% \usepackage{todonotes}

%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{0pt}
%\setlength{\floatsep}{0pt}
%\setlength{\textfloatsep}{1pt}
%\setlength{\dbltextfloatsep}{0pt}
%\setlength{\dblfloatsep}{0pt}
% \expandafter\def\expandafter\normalsize\expandafter{%
%      \normalsize
%      \setlength\abovedisplayskip{0pt}
%      \setlength\belowdisplayskip{0pt}
%      \setlength\abovedisplayshortskip{0pt}
%      \setlength\belowdisplayshortskip{0pt}
% }

% \usepackage{enumitem}
\usepackage{bm}

\makeatletter
\setlength{\@fptop}{0pt}
\makeatother

\usepackage{balance}

% % packages that might be useful for rebuttal
% \usepackage{savesym}
% \savesymbol{comment}
% \usepackage{changes}
% \restoresymbol{CHNG}{comment}
% \setaddedmarkup{\color{RoyalBlue}{#1}}
% \setdeletedmarkup{\color{red}{\sout{#1}}}
